Recognize Any Surgical Object: Unleashing the Power of Weakly-Supervised Data

We present RASO, a foundation model designed to Recognize Any Surgical Object, offering robust open-set recognition capabilities across a broad range of surgical procedures and object classes, in both surgical images and videos. RASO leverages a novel weakly-supervised learning framework that generates tag-image-text pairs automatically from large-scale unannotated surgical lecture videos, significantly reducing the need for manual annotations. Our scalable data generation pipeline gathers 2,200 surgical procedures and produces 3.6 million tag annotations across 2,066 unique surgical tags. Our experiments show that RASO achieves improvements of 2.9 mAP, 4.5 mAP, 10.6 mAP, and 7.2 mAP on four standard surgical benchmarks, respectively, in zero-shot settings, and surpasses state-of-the-art models in supervised surgical action recognition tasks. Code, model, and demo are available at https://ntlm1686.github.io/raso.

==> content/1_introduction.tex <==
\section{Introduction}
  Object recognition stands as a fundamental pillar in the field of computer vision, driving advancements that enable machines to interpret and interact with visual data effectively. Leveraging large-scale vision-language pretraining on abundant text-image pairs from the internet, models such as CLIP~\citep{radford2021learning_clip}, BLIP~\citep{li2022blip}, and Recognize Anything Model (RAM)~\citep{zhang2024recognize_ram} have demonstrated significant advancements in object detection and classification. Notably, models incorporating the RAM~\citep{zhang2024recognize_ram} have played a pivotal role in advancing grounded segmentation—a process where, given only an image as input, the model directly outputs label-segmentation pairs. Frameworks like Grounded SAM~\citep{ren2024grounded_sam} employ RAM to provide labels, then use models such as Grounding DINO~\citep{liu2023grounding_dino} to generate location anchors and finally apply the Segment Anything Model (SAM)~\citep{kirillov2023segany_sam} to obtain precise segmentation masks.

  Despite these breakthroughs,  surgical imaging has yet to benefit from strides achieved in these general computer vision tasks. For example, traditional models for surgical segmentation, such as Matis~\citep{ayobi2023matis} and S3Net~\citep{baby2023forks_s3net}, are constrained by their closed-set design, focusing on specific surgical procedures with a limited set of instruments or anatomical categories. This restricts their ability to generalize beyond the classes present in their training data. More recent models like SurgicalSAM~\citep{yue_surgicalsam} and MedSAM~\citep{MedSAM}, both fine-tuned versions of SAM, have demonstrated improved generalization in surgical segmentation tasks. However, MedSAM still requires manual inputs such as points or bounding boxes for segmentation, while SurgicalSAM, though independent of such inputs, is only fine-tuned on the EndoVis17~\citep{allan20192017_endovis17} and EndoVis18~\citep{allan20202018_endovis18} datasets, which are limited to the fixed set of classes (i.e., eleven classes). This narrow focus hampers these models' ability to generalize to the diverse range of instruments and procedures encountered in real-world surgical environments, including areas like surgical navigation, robotic assistance, and intraoperative decision-making.

  \input{figures/intro_eg}
  Therefore, we identify that a universal recognition model in the surgical domain would close the gap toward achieving surgical grounded segmentation. Such a model would not only handle segmentation tasks but also serve as a surgical foundation model.  Although grounded SAM has shown a multi-model expert system as an effective approach to grounded segmentation tasks, a major challenge is the scarcity of large-scale annotated surgical datasets, as manual annotation requires specialized expertise and is time-consuming. 
  
  To address these limitations and challenges, we present \textbf{R}ecognize \textbf{A}ny \textbf{S}urgical \textbf{O}bject (RASO) as a foundation model designed to bridge the gap between recognition and segmentation in surgical imaging as shown in Fig.~\ref{fig:intro_diff} (left). As an illustration, Fig.~\ref{fig:intro_eg} shows the comparison of various state-of-the-art methods in recognizing surgical objects when compared with human experts. We can see that RASO achieves much better performance than others and is closely aligned with clinician's annotations. Our major contributions to this work are as follows:
  \begin{itemize}
    \item \textit{RASO.} We present a novel open-set recognition model in the surgical domain, capable of recognizing a wide range of surgical objects from both images and videos. RASO incorporates a temporal-attention fusion layer to effectively capture the temporal relationships between video frames, improving the ability to capture surgical actions.

    \item \textit{Weakly-supervised Learning Framework.} We present a novel weakly-supervised learning framework that leverages unannotated surgical data to generate tag-image-text pairs automatically. This approach significantly reduces reliance on manual annotations, making it broadly applicable to other vertical domains where annotated data is scarce. The cost-efficiency of our approach allows us to train RASO within 8 hours using 8 A6000 GPUs.
    
    \item \textit{Weakly-supervised Data Generation Pipeline.} We introduce a scalable data generation pipeline that curates a comprehensive dataset from 2,200 unannotated surgical procedures, processing 901K images and 1.2M sentences. This pipeline generates 3.2M tag annotations from 2,066 unique surgical tags, all with minimal human intervention.

    \item \textit{Comprehensive Experiments.} We conduct extensive experiments, where RASO achieves improvements of 2.9 mAP, 4.5 mAP, 10.6 mAP, and 7.2 mAP across four standard surgical datasets in zero-shot settings. In the supervised setting, RASO also surpasses state-of-the-art (SOTA) models on the surgical action triplet recognition task. We validate the effectiveness of each component in our method through ablation studies.

  \end{itemize}
  


==> content/3_method.tex <==
\section{RASO}
\subsection{Architecture} \input{figures/method_arch} The architecture of RASO is built on RAM~\citep{zhang2024recognize_ram}. As shown in Fig.~\ref{fig:method_arch}, RASO consists of three key components: an image encoder, a spatial-temporal fusion layer, a tag decoder for surgical label prediction, and a text decoder for aligning visual and textual representations during pretraining. The core improvement over RAM is the introduction of a temporal fusion layer for efficient video recognition.

\textbf{Image Inference.} For image inputs, we utilize the Swin-Transformer~\citep{liu2021swin} to project the images to image features. We leverage the CLIP text encoder to embed the predefined tag list. The tag decoder then combines the visual features and the corresponding tag embeddings to predict logits for each tag. Finally, a predefined threshold is applied to identify the recognized objects.

\textbf{Video Inference \& Temporal-Attention Fusion Layer.} For video inputs, we uniformly sample $N$ frames and compute image embeddings using the same image encoder as for image inputs. The encoder generates frame-level features, denoted as $h_{\text{image}} \in \mathbb{R}^{T \times D}$, where $T$ represents the number of frames and $D$ is the feature dimension. These individual frame features are stacked along the temporal axis, resulting in a combined tensor $h_{\text{images}} \in \mathbb{R}^{N \times T \times D}$, capturing both spatial information and temporal progression. Afterward, the temporal-attention fusion layer is applied to aggregate temporal information across frames. Using a multi-head attention mechanism, the layer captures temporal dependencies between frames by reshaping and permuting the input into a format suitable for attention computation. The resulting tensor, $h_{\text{video}} \in \mathbb{R}^{T \times D}$, is seamlessly decoded using the same tag decoder as for image inputs, ensuring consistent prediction across both modalities. As shown in Section~\ref{sec:exp_ablation}, the temporal-attention fusion effectively captures dynamic information, particularly for categories that require temporal context to be correctly identified, such as surgical actions, thus enhancing video recognition performance.

\textbf{Pretraining.} During the pretraining phase, a text decoder reconstructs transcriptions from surgical lectures based on the visual features and predicted tags. This strengthens the alignment between visual content and textual information, improving the model’s ability to connect visual representations with semantic meaning. The text decoder is not used during inference.

\textbf{Open-Vocabulary Inference.} 
For unseen tags, the model uses the CLIP text encoder to generate embeddings, updating the tag embedding list accordingly. By leveraging the semantic relationships between known and unseen tags, the model can effectively generalize to new tags.

\subsection{Training}  The training process involves two stages: pretraining and fine-tuning.

\textbf{Stage 1: Pretraining.}
In this stage, we pretrain the model using 901K weakly supervised image-tag-text triplets extracted from WebSurg surgical lectures.
The core objective during pretraining is to align the visual features extracted from surgical videos with the corresponding textual information.
% These triplets align visual data with corresponding textual descriptions.
We keep the CLIP text encoder frozen and fine-tune the rest of the model for 10 epochs. 

\textbf{Stage 2: Fine-Tuning.}
In the fine-tuning phase, we fine-tune RASO with a mixture of image-tag and video-tag pairs. This combination enriched the model’s ability to generalize across diverse data formats. For zero-shot experiments, we exclusively relied on VLM-generated data as discussed in section~\ref{sec:engine}. We kept the CLIP text encoder frozen, fine-tune the rest of the model for 4 epochs.
% The fine-tuning phase builds on the pretraining by using both publicly available datasets and GPT-4o-generated image-tag pairs. Zero-shot experiments exclusively rely on the GPT-4o-generated data, yielding substantial improvements in transfer learning performance. The CLIP text encoder stays frozen while the rest of the model is fine-tuned for an 4 epochs.

\textbf{Discussion.} Our approach offers two major advantages: \textit{(i) Cost Efficiency.} We pretrained the model in less than 5 hours using 8 A6000 GPUs to process 901K samples over 10 epochs. Fine-tuning took 3 hours on the same hardware, demonstrating the scalability and resource efficiency of our method. \textit{(ii) Broad Applicability.} The method is applicable across other vertical domains where annotated data is scarce, but videos with voiceovers are abundant. For instance, medical instructional videos, which often include voiceovers, are ideal candidates for weakly supervised learning. This adaptability makes our method suitable for various fields with similar data structures.

\section{Weakly-supervised Data Generation} \label{sec:engine} \input{figures/method_pipeline}

To pretrain a robust foundation model for surgical object recognition, we curated a large-scale dataset capturing the complexity and diversity of surgical environments. As shown in Fig.~\ref{fig:method_data}, the dataset construction involved two main components: a \textit{label engine} and a \textit{data engine}. The label engine extracts relevant surgical tags from textual data, while the data engine aligns these tags with visual data from surgical lecture videos.

\subsection{Label Engine} Our goal was to build a comprehensive set of surgical tags encompassing organs, instruments, surgical actions, procedures, and phases. These tags form the model’s vocabulary, enabling it to recognize a wide variety of elements within surgical scenes. Our label engine consists of three parts:

\textbf{Surgical Entity Recognition.}
To curate a comprehensive set of static, domain-specific tags for surgical object recognition, we utilized spaCy’s biomedical model, \texttt{en\_core\_sci\_md}~\citep{neumann-etal-2019-scispacy}, to extract key entities such as anatomical structures, surgical instruments, and procedural terms from surgical lecture transcripts. This model, trained extensively on medical literature, excels in identifying Named Entities (NER) that are essential for understanding surgical contexts. By processing over 1.2 million sentences, we generated a wide-ranging set of relevant terms, capturing static objects like organs, tissues, and surgical tools, including scalpels and graspers. This process of entity recognition served as the backbone for developing a robust vocabulary, enabling the model to effectively recognize and differentiate critical elements within complex surgical scenes.


\textbf{Surgical Action Extraction.}
To capture the dynamic processes within surgical procedures, we employed SceneGraphParser~\citep{wu2019unified_sngparser} to extract detailed verb-noun pairs from surgical lecture transcripts. This parser identifies verb phrases representing actions and links them to their corresponding objects, such as surgical tools, anatomical structures, or tissues. Through this process, we automatically generate structured action triplets, such as $<$grasper dissects gallbladder$>$, where the verb ``dissects'' represents the action, ``grasper'' is the instrument acting, and ``gallbladder'' is the object being operated on. By extracting these action-object relationships, the model can understand both the activity taking place and the entities involved. This approach enriches the dataset with contextual information about the interactions between surgical tools and anatomical structures, which is crucial for accurately modeling the procedural flow and dynamics of surgical tasks.

\textbf{VLM Automated Annotation.} Recent studies~\citep{li2023comprehensive_gpteval1,cheng2023potential_gpteval2,hou2024gpteval3} have shown that models like GPT-4o can effectively recognize biomedical and surgical images. Leveraging this capability, we used GPT-4o to annotate 120K surgical images, generating 372K tag annotations. These auto-generated annotations enriched our dataset, providing additional weak supervision and reducing the need for manual labeling.

\subsection{Data Engine}

The data engine was developed to collect large-scale visual and textual data from surgical lecture videos. Specifically, we sourced 2,200 surgery procedures from platforms like WebSurg~\citep{websurg2024}, generating 901K images and 1.2 million sentences through WhisperX~\citep{bain2022whisperx}, which produced time-aligned transcriptions for each video. These videos were segmented into clips corresponding to individual sentences, and non-visual content, such as lecture slides, was filtered out using \textit{GPT-3.5-Turbo}~\citep{brown2020language_gpt3}. The filtered video clips, along with their transcriptions, were processed by the label engine to generate weakly supervised tag annotations. In total, the label engine utilized 2,066 tags (1,455 for pretraining and 611 for fine-tuning) to produce 3.6 million tag annotations. Frames were sampled from the annotated clips, and each frame was paired with the corresponding transcription and tags. This image-text-tag dataset formed the basis for pretraining, capturing diverse surgical environments, and reducing the need for manual annotation.


==> figures/intro_diff.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{assets/diff.pdf}
  \vspace{-0.5cm}
  \caption{RASO's Position in Grounded Surgical Segmentation Pipeline.}%Left: RASO's Position in Surgical Imaging. Right: Grounded Surgical Segmentation Pipeline. }
   \label{fig:intro_diff}
\end{figure}


==> figures/method_tags.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{assets/wordcloud_output.pdf}
  \caption{Word Cloud.} 
\label{fig:method_tags}
\vspace{-0.4cm}
\end{figure}

==> figures/method_training.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=.9\linewidth]{assets/training.pdf}
  \caption{RASO Training Pipeline.}
\label{fig:method_training}
\end{figure}

==> tables/ablation.tex <==
\begin{table}[ht]
\centering
\caption{Ablation study results with check marks representing components used in each setup.}
\begin{tabular}{@{}lcccccc@{}}
\toprule
& Pretrain & GPT-4o & CholecT50 & Cholec80 & Endovis18 & GraSP \\ 
\midrule
\multirow{3}{*}{Zero-shot} & \textcolor[rgb]{0,0.8,0}{$\checkmark$} & \textcolor[rgb]{0,0.8,0}{$\checkmark$}  & 22.6 & 37.8 & 58.8 & 20 \\ 
& \textcolor[rgb]{0,0.8,0}{$\checkmark$}  &  & 20.6 & 25 & 53.3 & 16.4 \\ 
&  & \textcolor[rgb]{0,0.8,0}{$\checkmark$}  & - & - & - & - \\ 
\midrule
& Pretrain & GPT-4o & Instrument & Verb & Target & All \\ 
\midrule
\multirow{3}{*}{Supervised} & \textcolor[rgb]{0,0.8,0}{$\checkmark$}  &  & 88.3 & 63.4 & 40.5 & 57.5 \\ 
& \textcolor[rgb]{0,0.8,0}{$\checkmark$}  & \textcolor[rgb]{0,0.8,0}{$\checkmark$}  & - & - & - & - \\ 
&  &  & 83.3 & 59 & 40 & 54.8 \\ 
\midrule
& Avg Pooling & Temporal Attention & Instrument & Verb & Target & All \\ 
\midrule
\multirow{2}{*}{Video} & \textcolor[rgb]{0,0.8,0}{$\checkmark$}  & & 90.3 & 68.5 & 41.7 & 60.1 \\ 
& & \textcolor[rgb]{0,0.8,0}{$\checkmark$}  & 88.9 & 74.5 & 41 & 61.3 \\ 
\bottomrule
\end{tabular}
\end{table}
